Using GXWeb for Theorem Proving and Mathematical Modelling

GXWeb is the free browser based version of the symbolic geometry software Geometry Expressions. We demonstrate its use in an educational setting with examples from theorem proving, mathematical modelling and loci and envelopes.

==> eptcsdata.tex <==
\providecommand{\firstpage}{38}
\providecommand{\publicationstatus}{P. Quaresma and Z. Kov{\'a}cs (Ed.): Automated Deduction\\ in Geometry 2023 (ADG 2023).\\
EPTCS 398, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.398.7}{10.4204/EPTCS.398.7}}
\pdfoutput=1

